Model rejection and parameter reduction via time series

We show how a graph algorithm for finding matching labeled paths in pairs of labeled directed graphs can be used to perform model validation for a class of dynamical systems including regulatory network models of relevance to systems biology. In particular, we extract a partial order of events describing local minima and local maxima of observed quantities from experimental time-series data from which we produce a labeled directed graph we call the pattern graph for which every path from root to leaf corresponds to a plausible sequence of events. We then consider the regulatory network model, which can be itself rendered into a labeled directed graph we call the search graph via techniques previously developed in computational dynamics. Labels on the pattern graph correspond to experimentally observed events, while labels on the search graph correspond to mathematical facts about the model. We give a theoretical guarantee that failing to find a match invalidates the model. As an application we consider gene regulatory models for the yeast S. cerevisiae.

==> figures/network_bad.tex <==
\begin{figure}[h!]
  \begin{center}
    \begin{tikzpicture}[main node/.style={rectangle,fill=white!20,draw,font=\sffamily\normalsize},scale=1.6]
      \node[main node] (SWI) at (0,0) {NDD1};
      \node[main node] (HCM) at (1.5,0) {HCM1};
      \node[main node] (NDD) at (3,0) {SWI4};
      \node[main node] (YOX) at (0,1) {YOX1};

      \path[->,>=angle 90,thick]
      (YOX) edge[-|,shorten <= 3pt, shorten >= 3pt, bend left] node[] {} (SWI)
      (SWI) edge[->,shorten <= 3pt, shorten >= 3pt, bend left] node[] {} (YOX)
      (SWI) edge[->,shorten <= 3pt, shorten >= 3pt] node[] {} (HCM)
      (HCM) edge[->,shorten <= 3pt, shorten >= 3pt] node[] {} (NDD)
      (NDD) edge[->,shorten <= 3pt, shorten >= 3pt, bend left] node[] {} (SWI)
      ;

      \end{tikzpicture}
    \end{center}
  \caption{A hypothetical regulatory network for the data in Figure~\ref{fig:dataset} which our methodology invalidates.}
  \label{fig:regnetwork_invalidate}
\end{figure}

